Characterizing Event-themed Malicious Web Campaigns: A Case Study on War-themed Websites

Cybercrimes such as online scams and fraud have become prevalent. Cybercriminals often abuse various global or regional events as themes of their fraudulent activities to breach user trust and attain a higher attack success rate. These attacks attempt to manipulate and deceive innocent people into interacting with meticulously crafted websites with malicious payloads, phishing, or fraudulent transactions. To deepen our understanding of the problem, this paper investigates how to characterize event-themed malicious website-based campaigns, with a case study on war-themed websites. We find that attackers tailor their attacks by exploiting the unique aspects of events, as evidenced by activities such as fundraising, providing aid, collecting essential supplies, or seeking updated news. We use explainable unsupervised clustering methods to draw further insights, which could guide the design of effective early defenses against various event-themed malicious web campaigns.

==> limitation.tex <==
%\vspace{-0.7em}
%\subsection{Discussion and Insights}

%\footnote{incorporate this subsection into the previous section}
%Theme threat attacks are becoming a matter of grave concern for the researchers as new kinds of mass events are very frequent this days.
%With our initial hypothesis on the propagation of malicious activities through Russia-Ukraine war themed websites, we come up with a clustering based identification of such attack using Russia-Ukraine war related websites domain. 
%By following a well structured methodology, first we have created a pipeline to solve the problem. Then, we have been able to extract some relevant features which helped us to distinguish the clusters properly. Finally, we have characterized all the five clusters with data driven analysis and a third party website evaluator. 

\label{sec:limit}
\input{limitation}
Our case study has limitations to be addressed in future studies. First, we focus on studying event-themed campaigns at their early stage. However, we did not quantify the notion of {\em early stage} (e.g., should the first week of a campaign considered early stage?). This is important because datasets of an event-themed malicious web campaign would evolve with time and this early stage may also vary based on the gravity of the event. 
%, As we have started our research lately after the initial collection of domain names, a significant number of websites were not live, which hinders our capability to analyze these websites in details. 
Second, the website domain names in our dataset only contain the word `Ukraine' or `Ukranian' but not necessarily `Russia' or `Russian'. This means that the dataset may have missed other relevant domains. 
%{\color{blue} Third, the content features are extracted from the final landing page, so the content of the other pages was not explored and not included in the feature list.} 
Third, our manual analysis to understand the quality of the results is conducted on a small number of websites because there is no ground truth available, and thus may make the website structure not relevant with their initial state when the feature extraction was performed. Fourth, we did not investigate whether any of the websites used cloaking techniques \cite{CrawlPhish_Oest_sp22_cloaking}, which may lead to the identification of other patterns. Fifth, during the feature extraction process from website contents, we only consider English language-based keywords but there might be keywords in other languages (e.g., Russian, Ukrainian, or other minor languages in the region). 

